Asymptotic behaviour of the third Painlev\'e transcendents in the space of initial values

We study the asymptotic behaviour of the solutions of the generic ($D_6^{(1)}$-type) third Painlev\'e equation in the space of initial values as the independent variable approaches infinity (or zero) and show that the limit set of each solution is compact and connected. Moreover, we prove that any solution with essential singularity at infinity has an infinite number of poles and zeroes, and similarly at the origin.

==> A-p3resolution/notation.tex <==
In this appendix, we collect the notation for base points, provide the charts in which they are defined and their coordinates in these charts, and give the relationships between constants used in the paper. 

\renewcommand{\arraystretch}{2}
\begin{longtable}[h]{|c|l|c|}
\hline
base point & coordinate system & coordinates\\
\hline
\endhead
\hline
\endfoot
  $b_1$ & $(y_{02},z_{02})=(\dfrac1y,\dfrac{z}{y})$ & $(0,0)$ 
  \\
  $b_2$ & $(y_{03},z_{03})=(\dfrac1{z},\dfrac{y}{z})$ & $(0,0)$  
  \\
  $b_3$ & $(y_{12},z_{12})=(y_{02},\dfrac{z_{02}}{y_{02}})=(\dfrac1y,z)$ & $(0,\sqrt{4\gamma})$
  \\
  $b_4$ & $(y_{12},z_{12})=(y_{02},\dfrac{z_{02}}{y_{02}})=(\dfrac1y,z)$ & $(0,-\sqrt{4\gamma})$
  \\  
  $b_5$ & $(y_{22},z_{22})=(y_{03},\dfrac{z_{03}}{y_{03}})=(\dfrac1z,y)$ & $(0,0)$
  \\  
  $b_6$ & $(y_{32},z_{32})=(y_{12},\dfrac{z_{12}-\sqrt{4\gamma}}{y_{12}})=(\dfrac1{y},y(z-\sqrt{4\gamma}))$ 
  & $(0,\dfrac{2\alpha}{x\sqrt{\gamma}})$
  \\
   $b_7$ & $(y_{42},z_{42})=(y_{12},\dfrac{z_{12}+\sqrt{4\gamma}}{y_{12}})=(\dfrac1{y},y(z+\sqrt{4\gamma}))$ 
  & $(0,-\dfrac{2\alpha}{x\sqrt{\gamma}})$
  \\
   $b_8$ & $(y_{51},z_{51})=(\dfrac{y_{22}}{z_{22}},z_{22})=(\dfrac1{yz},y)$ & $(0,0)$
  \\  
   $b_9$ & $(y_{81},z_{81})=(\dfrac{y_{51}}{z_{51}},z_{51})=(\dfrac1{y^2z},y)$ & $(-\dfrac1{4\delta_1},0)$
  \\   
   $b_{10}$ & 
   $(y_{91},z_{91})=(\dfrac{1}{z_{81}}(y_{81}+\dfrac{1}{4\delta_1}),z_{81})=(\dfrac1y(\dfrac1{y^2z}+\dfrac1{4\delta_1}),y)$ & $(-\dfrac{\beta_1+4\delta_1}{8x\delta_1^3},0)$
  \\   
   $b_{11}$ & $(y_{52},z_{52})=(y_{22},\dfrac{z_{22}}{y_{22}})=(\dfrac1z,yz)$ & $(0,-\dfrac{2\beta_1}{\delta_1 x})$
\end{longtable}

Note that the constants used throughout the paper are related as follows.
\begin{align*}
&\delta_1=i\sqrt{\delta},
\\
&\beta_1=\beta-2\delta_1.
\end{align*}


